Local fraction in Static Causal Orders

In this Letter, we introduce a notion of local fraction for experiments taking place against arbitrary static causal backgrounds -- greatly generalising previous results on no-signalling scenarios -- and we explicitly formulate a linear program to compute this quantity. We derive a free characterisation of causal functions which allows us to efficiently construct the matrices required to perform concrete calculations. We demonstrate our techniques by analysing the local fraction of a novel example involving two Bell tests in interleaved causal order.

==> eptcs-packages.tex <==
\usepackage{amsmath}
\usepackage{amssymb} %
\usepackage{bbold} %
\usepackage{bbm} %
\usepackage{amsthm} %
\usepackage{stmaryrd} %
\usepackage{etoolbox} %
\usepackage{xparse}
\usepackage{pgffor}


\usepackage[utf8]{inputenc} %
\usepackage{textgreek} %
\usepackage{relsize} %
\usepackage{microtype} %
\usepackage{ulem} %
\usepackage[compress]{cite} %
\usepackage{csquotes} %
\usepackage{setspace} %
\usepackage{scalerel}


\usepackage{graphicx} %
\usepackage[usenames,dvipsnames]{xcolor} %
\usepackage{tikzit} %
\usepackage{stackengine}
\usepackage{circuitikz} %
\usetikzlibrary{
    arrows,
    shapes,
    decorations,
    intersections,
    backgrounds,
    positioning,
    circuits.ee.IEC
    }
\input{thesis.tikzstyles}




\definecolor{evred}{rgb}{0.996, 0.403, 0.537}
\definecolor{evgreen}{rgb}{0.501, 1.0, 0.505}
\definecolor{evblue}{rgb}{0.2, 0.588, 1.0}




\usepackage[frozencache]{minted} %


\usemintedstyle{default}
\setminted[python]{
bgcolor=lightgray!10,
xleftmargin=2mm,
fontsize=\footnotesize,
frame=lines,
linenos,
python3=true}
\setminted[text]{
bgcolor=lightgray!10,
xleftmargin=2mm,
fontsize=\footnotesize}

